ST-ExpertNet: A Deep Expert Framework for Traffic Prediction

Recently, forecasting the crowd flows has become an important research topic, and plentiful technologies have achieved good performances. As we all know, the flow at a citywide level is in a mixed state with several basic patterns (e.g., commuting, working, and commercial) caused by the city area functional distributions (e.g., developed commercial areas, educational areas and parks). However, existing technologies have been criticized for their lack of considering the differences in the flow patterns among regions since they want to build only one comprehensive model to learn the mixed flow tensors. Recognizing this limitation, we present a new perspective on flow prediction and propose an explainable framework named ST-ExpertNet, which can adopt every spatial-temporal model and train a set of functional experts devoted to specific flow patterns. Technically, we train a bunch of experts based on the Mixture of Experts (MoE), which guides each expert to specialize in different kinds of flow patterns in sample spaces by using the gating network. We define several criteria, including comprehensiveness, sparsity, and preciseness, to construct the experts for better interpretability and performances. We conduct experiments on a wide range of real-world taxi and bike datasets in Beijing and NYC. The visualizations of the expert's intermediate results demonstrate that our ST-ExpertNet successfully disentangles the city's mixed flow tensors along with the city layout, e.g., the urban ring road structure. Different network architectures, such as ST-ResNet, ConvLSTM, and CNN, have been adopted into our ST-ExpertNet framework for experiments and the results demonstrates the superiority of our framework in both interpretability and performances.

==> Preliminary.tex <==
\begin{definition}\label{def:flow}
	\textbf{Inflow and outflow~\cite{zhang2016dnn}}.
	Let ~$\mathbb{P}$ ~be the set of trajectories in the $t^{th}$ time interval. For a grid of inflow and outflow matrix at $i$ rows and $j$ columns, the
	inflow $g_{t}^{i n, i, j}$ and outflow $g_{t}^{o u t, i, j}$ of the crowds are defined as 
	\begin{align*}
		g_{t}^{i n, i, j} &=\sum_{T r \in \mathbb{P}}\left|\left\{k>1 \mid v_{k-1} \notin(i, j) \wedge v_{k} \in(i, j)\right\}\right| \\
		g_{t}^{o u t, i, j} &=\sum_{T r \in \mathbb{P}}\left|\left\{k \geq 1 \mid v_{k} \in(i, j) \wedge v_{k+1} \notin(i, j)\right\}\right|
	\end{align*}
	where, $T r: v_{1} \rightarrow v_{2} \rightarrow \cdots \rightarrow v_{|T r|}$ is a single trajectory in $\mathbb{P}$.
	$v_{k}\in(i, j)$ means that the trajectory $v_{k}$ coordinate at the region of $g_{t}^{i, j}$. $| \cdot |$  denotes cardinality of a set. \\
\end{definition}
\begin{figure}
	\centering
	\includegraphics[width=1\linewidth]{image/formulation}
	\caption{Schematic of our framework. We intend to build a set of models, which can automaticly disentangle the feature pattern (e.g. working, entertaining, commuting and commercial ect) from input and predict the future flow prediction by the weighted summation of each part. }
	\label{fig:formulation}
\end{figure}

\begin{definition}\label{def:flowpred}
	\textbf{Flow prediction}.
	Given the historical observations 
	$G_t=\left\{g_{t^{\prime}} \mid t^{\prime} \in[t-n+1, t]\right\}$
	, predict future $m$ steps flow $Y_{t+1:t+m}$.
	\begin{equation}
		\Phi: G_t \rightarrow Y_{t+1:t+m}\label{equ:flow_pred}
	\end{equation}
	where $\Phi$ as neural network and $n$ denotes the length of the input time interval, $G_t \in \mathbb{R}^{2n \times h \times w}$ and $h, w$ denote the height and width of region size.\\
\end{definition}
%\begin{definition}\label{def:selfexp}
%	\textbf{Self-explaining models~\cite{alvarez2018towards}}.
%	 Let $h(x): \mathcal{X} \rightarrow \mathcal{Z} \subset \mathbb{R}^{k}$, where $\mathcal{Z}$ is some space of interpretable atoms.  Alternatives for $h(\cdot)$ include:
%	 \begin{itemize}
%	 	\item 
%	 \end{itemize}
%	  (i) subset aggregates of the input (e.g., with $h(x)=A x$ for a boolean mask matrix $A$ ), (ii) predefined, pre-grounded feature extractors designed with expert knowledge (e.g., filters for image processing), (iii) prototype based concepts, e.g. $h(x)_{i}=\left\|x-\xi_{i}\right\|$ for some $\xi_{i} \in \mathcal{X}$ [12], or (iv) learnt representations with specific constraints to ensure grounding [19]. Naturally, we can let $h(x)=x$ to recover raw-input explanations if desired. The generalized model is now:
%	\begin{align}
%		f(x)=\theta(x)^{\top} h(x)=\sum_{i=1}^{k} \theta(x)_{i} h(x)_{i}
%	\end{align}
%\end{definition}




==> abstract.tex <==


%In this paper, we propose  that can modeling 
